GEANT4 simulation of a new range verification method using delayed gamma spectroscopy of a Mo-92 marker

In this work, we propose a novel technique for in-vivo proton therapy range verification. This technique makes use of a small hadron tumour marker, $^{92}$Mo, implanted at a short known distance from the clinical treatment volume. Signals emitted from the marker during treatment can provide a direct measurement of the proton beam energy at the marker's position. Fusion-evaporation reactions between the proton beam and marker nucleus result in the emission of delayed characteristic $\gamma$ rays, which are detected off-beam for an improved signal-to-noise ratio. In order to determine the viability of this technique and to establish an experimental setup for future work, the Monte Carlo package GEANT4 was used in combination with ROOT to simulate a treatment scenario with the new method outlined in this work. These simulations show that analyzing the intensity of delayed $\gamma$ rays produced from competing reactions yields a precise measurement of the range of the proton beam relative to the marker, with sub-millimeter uncertainty.

==> README <==
# harvard family of bibliographic styles
# Copyright 1994 - Peter Williams pwil3058@bigpond.net.au
#
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
# 
# The Current Maintainers of this work are Peter Williams and Thorsten Schnier.
#
# This work consists of all files listed in manifest.txt.
#
# Licence notice added on behalf of Peter Williams and Thorsten Schnier
# by Clea F. Rees 2009/01/30.

This is version 2.0.5 of the harvard family of bibliographic styles.
It is a bug fix of 2.0 which was a major rewrite to bring the sty file into
line with the new latex described in ``The LaTeX Companion''.  Due to the
efforts of Thorsten Schnier (thorsten@archsci.arch.su.edu.au) it incorporates
support for the LaTeX to html translator by Nikos Drakos
(nikos@cbl.leeds.ac.uk).

It includes a fixes by Berwin A. Turlach (berwin@alphasun.anu.edu.au) for
problems with \AtBeginDocument introduced in the latest version of LaTeX2e
and problems with the \nocite command.

A new style apsr.bst (American Political Science Review) is enclosed
courtesy of Nathaneil L. Beck (nbeck@weber.ucsd.edu)

NB.  The file harvard.sty makes considerable use of features in the new latex
that were not present in latex version 2.09 and is, therefore, not compatible
with that version.  However, the *.bbl files produced by the various bst files
should be still useable with latex version 2.09.

The following files are enclosed.

  README	- This file
  INSTALL	- Installation instructions
  Makefile	- Makefile for installation
  harvard.ps	- Postscript version of the documentation
  harvard.tex	- LaTeX source for the documentation
  harvard.bib	- BibTeX database file for the documentation
  doc_Makefile	- Makefile for documentation
  harvard.sty	- LaTeX style file for harvard bibliographic style
  harvard.perl	- LaTeX2html style file for harvard bibliographic style
  agsm.bst	- harvard BibTeX style file to satisfy the requirements
		  of the Australian Government Style Manual
  dcu.bst	- harvard BibTeX style file to satisfy the requirements
		  of the Design Computing Unit, Sydney University
  <other>.bst	- various style files contributed by users

Online documentation is available via the WWW at:

HREF="http://www.arch.su.edu.au/~peterw/latex/harvard/"

